Smoothing Meets Perturbation: Unified and Tight Analysis for Nonconvex-Concave Minimax Optimization

This paper studies smooth nonconvex-concave minimax optimization and two acceleration mechanisms for single-loop first-order methods: dual perturbation and smoothing. Although both techniques improve convergence guarantees, their relative advantages remain unclear due to the distinction between game stationarity (GS) and optimization stationarity (OS). We provide a tight characterization of their iteration complexities under both notions. We show that smoothing accelerates convergence to both GS and OS, whereas dual perturbation improves the rate only for GS and does not accelerate OS. Matching lower bounds based on hard instances establish the tightness of these rates. Motivated by this separation, we propose Perturbed Smoothed GDA, a single-loop method combining both techniques. It improves the complexity for GS over existing single-loop methods while preserving the state-of-the-art rate for OS, and further admits asymptotic convergence to 0-GS, which is not available for vanilla Smoothed GDA.

==> def_jiajin.tex <==
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage[in]{fullpage}



%\usepackage{hyperref}      % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography

\usepackage{subcaption}

\usepackage{mathrsfs}

% Page Formatting
% \textheight 8.5in
% \addtolength{\topmargin}{-0.4in}
% \addtolength{\oddsidemargin}{-0.7in}
% \addtolength{\textwidth}{1.35in}

% for colorful table
\usepackage[table,xcdraw]{xcolor}
% for color
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{amber}{rgb}{1.0, 0.75, 0.0}
\definecolor{burntorange}{rgb}{0.8, 0.33, 0.0}
\definecolor{dimgray}{rgb}{0.41, 0.41, 0.41}

% \usepackage[pdfencoding=auto, psdextra, colorlinks]{hyperref} 
\usepackage[pagebackref = true,linkcolor={red!80!black},citecolor={blue!70!black}, urlcolor={blue!70!black},colorlinks, breaklinks]{hyperref}
%\usepackage{nicematrix}
% tikz begin
\usepackage{tikz}
\usetikzlibrary{fit}
\tikzset{%
	%highlight/.style={rectangle,blend mode = multiply,fill=blue!20,fill,rounded corners = 0.3 mm,inner sep=1pt}
	highlight/.style={rectangle,blend mode = multiply,draw=blue!90!black,thick,rounded corners = 0.3 mm,inner sep=0.5pt}
}
\newcommand{\markEle}[2]{\tikz[remember picture,overlay] \node[highlight, fit = (#1-#2-medium) (#1-#2-medium)] {};}
% tikz end


\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

\usepackage{amsmath,amssymb,amsthm}
\usepackage[ruled,linesnumbered]{algorithm2e}
% \usepackage{algorithm,algorithmicx,algpseudocode}
% the following set font for mathbb
\usepackage{bbold}
% dsfont
\usepackage[sans]{dsfont}
% clever ref
% \usepackage[numbers]{natbib}
%\def\citep\cite
%\usepackage{natbib}
% \usepackage{cleveref}

% for circle number \ding{172} for 1
\usepackage{pifont}

% for colors
%\usepackage{xcolor}
% for advanced theorem tools and restatable claims
\usepackage{thmtools}
\usepackage{thm-restate}

\usepackage{multirow}

% following package help make the table full textwidth
\usepackage{tabularx}

% for straight quote, use: \textquotesingle
\usepackage{textcomp}

\usepackage[shortlabels]{enumitem}
%\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
%\setenumerate{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
%\setlist[itemize]{itemsep=0mm}
%\setlist[enumerate]{itemsep=0mm}
%\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
%\setlength{\parindent}{0pt}

%\usepackage{nicematrix}


% operate norm
%\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1\right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

% <-- theorem related begin -->
%\declaretheorem[thmbox=L]{thm}
%\declaretheorem[name=Theorem,within=section,shaded={rulecolor=gray,rulewidth=1pt, bgcolor={rgb}{1,1,1}}]{theorem}
\usepackage{thmtools}

\renewcommand{\qedsymbol}{$\blacksquare$}
% \declaretheorem{theorem}
% \declaretheorem{corollary}
% \declaretheorem{lemma}
% \declaretheorem{proposition}
% \declaretheorem{observation}
% \declaretheorem{fact}
% \declaretheorem{algorithm}

\declaretheoremstyle[qed=$\square$,parent=section]{definitionwithend}
\declaretheorem[style=definitionwithend]{corollary}
\declaretheorem[style=definitionwithend]{theorem}
\declaretheorem[style=definitionwithend]{proposition}
\declaretheorem[style=definitionwithend]{definition}
\declaretheorem[style=definitionwithend]{assumption}
\declaretheorem[style=definitionwithend]{example}
\declaretheorem[style=definitionwithend]{remark}
\declaretheorem[style=definitionwithend]{question}
\declaretheorem[style=definitionwithend]{lemma}
\declaretheorem[style=definitionwithend]{fact}
% \declaretheorem[name=Theorem,within=section,style=definitionwithend]{thm}
% \declaretheorem[name=Lemma,sibling=thm,style=definitionwithend]{lemma}
% \declaretheorem[name=Corollary,sibling=thm,style=definitionwithend]{coro}
% \declaretheorem[name=Example,sibling=thm,style=definitionwithend]{exam}
% \declaretheorem[name=Remark,sibling=thm,style=definitionwithend]{rmk}
% \declaretheorem[name=Definition,sibling=thm,style=definitionwithend]{defi}
% \declaretheorem[name=Claim,sibling=thm,style=definitionwithend]{claim}
% \declaretheorem[name=Conjecture,sibling=thm,style=definitionwithend]{conjecture}
% \declaretheorem[name=Assumption,sibling=thm,style=definitionwithend]{ass}
% \declaretheorem[name=Fact,sibling=thm,style=definitionwithend]{fact}
% \declaretheorem[name=Proposition,sibling=thm,style=definitionwithend]{prop}
% <-- theorem related end -->

% tikz begin
\usepackage{tikz}
\usetikzlibrary{shadows}
\usetikzlibrary{arrows,positioning} 
\def\arraystretch{1.5}
\setlength\tabcolsep{2mm}
\setlength\arrayrulewidth{0.8pt}
\newcommand\hfilll{\hspace{0pt plus 1filll}}
% tikz end
%%%%%%%%%%%%%%%%%%

% for underline
% underline
\usepackage{contour}
\usepackage[normalem]{ulem}

\renewcommand{\ULdepth}{1.8pt}
\contourlength{0.8pt}

\newcommand{\myuline}[1]{%
	\uline{\phantom{#1}}%
	\llap{\contour{white}{#1}}%
}
% underline end

% equation numbering with section
\numberwithin{equation}{section}

\setlength{\tabcolsep}{3 pt}


\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut

% for bold greek
\usepackage{bm}

% for warp figure
\usepackage{wrapfig}



% add comments
%\newcommand\tltodo[1]{\textcolor{blue}{[TL: #1]}}
% \definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
% \newcount\Comments
% \Comments=1 
% \newcommand{\kibitz}[2]{\ifnum\Comments=1{\textcolor{#1}{\textsf{\footnotesize #2}}}\fi}
% \newcommand{\Jiajin}[1]{\kibitz{magenta}{[Jiajin: #1]}}
%\author{}
\usepackage{authblk}
% \renewcommand*{\Authsep}{, }
\renewcommand*{\Authand}{, }
\renewcommand*{\Authands}{, }
\renewcommand*{\Affilfont}{\normalsize}
%\renewcommand*{\Authfont}{\bfseries}    % make author names boldface    
\setlength{\affilsep}{1em}   % set the space between author and affiliation

% definition
% Hotkeys
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\imply}{\Rightarrow}
\newcommand{\ifaof}{\Leftrightarrow}
\newcommand{\limto}{\rightarrow}
\newcommand{\del}{\partial}
\newcommand{\bz}{\mathbf 0}
\newcommand{\PP}{\mathbb P}
\newcommand{\QQ}{\mathbb Q}
\newcommand{\EE}{\mathbb E}
\newcommand{\R}{\mathbb R}
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\Y}{\mathbb Y}
\newcommand{\E}[1]{{\mathbb E}\left[ #1 \right]}
\newcommand{\mc}{\mathcal}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eps}{\varepsilon}
\newcommand{\Let}{\triangleq}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\FOAM}{FOAM}
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\res}{Res}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\st}{s.t.}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}




% for def over equal
\newcommand{\defequal}{\overset{\text{\tiny{def}}}{=}}
\newcommand{\commentColor}{blue!90!black}

% \let\oldComment\Comment
% \renewcommand{\Comment}[1]{\oldComment{\textcolor{\commentColor}{#1}}}


\def\O#1{\text{\ding{\the\numexpr#1+171}}}

\usepackage{threeparttable}
\allowdisplaybreaks[4] % spread setup 


\def\keywords{\vspace{1.5em}
{\textbf{Keywords}:\,\relax%
}}
\def\endkeywords{\par}

% \hypersetup{
%     pagebackref=true,
%     colorlinks=true,
%     breaklinks,
%     linkcolor={red!80!black},
%     citecolor={blue!70!black},
%     urlcolor={blue!70!black}
% }
% Font Shortcuts
\newcommand{\mb}{\mathbf}
\newcommand{\bs}{\boldsymbol}
% \newcommand{\mc}{\mathcal}
\newcommand{\bb}{\mathbb}
\newcommand{\bbm}{\mathbbm}
\newcommand{\mf}{\mathfrak}

%Letters in different typefaces
%\newcommand{\A}{\mathbb{A}}
\def\A{{\mathbb{A}}}
\def\B{{\mathbb{B}}}
\def\C{{\mathbb{C}}}
\def\D{{\mathbb{D}}}
\def\E{{\mathbb{E}}}
\def\F{{\mathbb{F}}}
\def\G{{\mathbb{G}}}
\def\H{{\mathbb{H}}}
\def\I{{\delta}}
\def\J{{\mathbb{J}}}
\def\K{{\mathbb{K}}}
\def\L{{\mathbb{L}}}
\def\M{{\mathbb{M}}}
\def\N{{\mathbb{N}}}
\def\O{{\mathbb{O}}}
\def\P{{\mathbb{P}}}
\def\Q{{\mathbb{Q}}}
\def\R{{\mathbb{R}}}
\def\S{{\mathbb{S}}}
\def\T{{\mathbb{T}}}
\def\U{{\mathbb{U}}}
\def\V{{\mathbb{V}}}
\def\W{{\mathbb{W}}}
\def\X{{\mathbb{X}}}
\def\Y{{\mathbb{Y}}}
\def\Z{{\mathbb{Z}}}

\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def \cR{{\cal \cR}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

\def\a{{\mathbf a}}
\def\b{\bm{b}}
\def\c{{\mathbf c}}
\def\d{\bm{d}}
\def\e{{\mathbf e}}
\def\f{{\mathbf f}}
\def\g{{\mathbf g}}
\def\h{\bm{h}}
\def\i{{\mathbf i}}
\def\j{{\mathbf j}}
\def\k{{\mathbf k}}
\def\l{{\mathbf l}}
\def\m{{\mathbf m}}
\def\n{{\mathbf n}}
\def\o{{\mathbf o}}
%\def\p{{\mathbf p}}
\def\p{\bm{p}}
%\def\q{{\mathbf q}}
\def\q{\bm{q}}
\def\r{{\mathbf r}}
\def\s{{\mathbf s}}
\def\t{{\mathbf t}}
\def\u{{\mathbf u}}
\def\v{\bm{v}}
\def\w{{\mathbf w}}
%\def\x{{\mathbf x}}
\def\x{\bm{x}}
%\def\y{{\mathbf y}}
\def\y{\bm{y}}
\def\z{\bm{z}}
\def\bz{{\mathbf 0}}
\def\lbd{{\lambda}}
\def\1{{\mathbf 1}}
\def\prox{{\rm{prox}}}
\def\proxbar{\overline{\textrm{prox}}}
\def\dist{{\operatorname{dist}}}
\def\bx{\bm{x}}
\def\by{\bm{y}}
\def\intm{{\rm int}}

\newcommand{\tO}{{\tilde{\mathcal O}}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\rank}{\mathrm{rank} }
\newcommand{\blam}{{\boldsymbol\lambda}}
\newcommand{\bga}{{\boldsymbol\gamma}}
\newcommand{\bmu}{{\boldsymbol\mu}}
\newcommand{\bnu}{{\boldsymbol\nu}}
\newcommand{\bbt}{{\boldsymbol\beta}}
\newcommand{\bro}{{\boldsymbol\rho}}


